A Uniform Catalog of Molecular Clouds in the Milky Way

The all-Galaxy CO survey of Dame, Hartmann, & Thaddeus (2001) is by far the most uniform, large-scale Galactic CO survey. Using a dendrogram-based decomposition of this survey, we present a catalog of 1064 massive molecular clouds throughout the Galactic plane. This catalog contains $2.5 \times 10^8$ solar masses, or $25^{+10.7}_{-5.8} \%$ of the Milky Way's estimated H$_2$ mass. We track clouds in some spiral arms through multiple quadrants. The power index of Larson's first law, the size-linewidth relation, is consistent with 0.5 in all regions - possibly due to an observational bias - but clouds in the inner Galaxy systematically have significantly (~ 30%) higher linewidths at a given size, indicating that their linewidths are set in part by Galactic environment. The mass functions of clouds in the inner Galaxy versus the outer Galaxy are both qualitatively and quantitatively distinct. The inner Galaxy mass spectrum is best described by a truncated power-law with a power index of $\gamma=-1.6\pm0.1$ and an upper truncation mass $M_0 = (1.0 \pm 0.2) \times 10^7 M_\odot$, while the outer Galaxy mass spectrum is better described by a non-truncating power law with $\gamma=-2.2\pm0.1$ and an upper mass $M_0 = (1.5 \pm 0.5) \times 10^6 M_\odot$, indicating that the inner Galaxy is able to form and host substantially more massive GMCs than the outer Galaxy. Additionally, we have simulated how the Milky Way would appear in CO from extragalactic perspectives, for comparison with CO maps of other galaxies.

==> discussion.tex <==
%!TEX root = manuscript.tex

% In this section we discuss how our results relate to other studies and the overall understanding of GMCs in galaxies.

% \subsection{Comparison to Galactic studies}
% \label{sec:discuss_galactic}

% % This study is unique among all previous studies of molecular clouds in the Galaxy in that it is a systematic decomposition of CO emission throughout the entire Galactic plane into clouds.

% Much here will connect with the Heyer \& Dame review, and the various Galactic studies mentioned throughout the paper. 

% \begin{enumerate}
% 	\item comparing the total mass found in each quadrant to comparable surveys. e.g., compare 1st quadrant to \citet{dame86}, \citet{scoville87}; compare outer Galaxy to \citet{sodroski91}; compare 4th quadrant to \citet{garcia14}.
% 	\item Comparing the size-linewidth slopes to the above previous Galactic studies
% 	\item comparing the mass function to the above studies.
% \end{enumerate}

% \subsection{Comparison to Extragalactic studies}
% \label{sec:discuss_extragalactic}

% Much here will connect with the \citet{fukui10} extragalactic review, as well as the \citet{colombo14} paper.
% Especially will focus on similarities and differences between this and the Colombo paper, esp. on how the mass function varies with region.

% \subsection{Implications for GMCs in galaxies}
% \label{sec:discuss_GMCs}

% I will discuss what the implications of the mass function's regional dependence is.
% GMC formation/destruction physics, with citations (some from Colombo, some from Kennicutt 2012 review).
